Busemann functions, geodesics, and the competition interface for directed last-passage percolation

In this survey article we consider the directed last-passage percolation model on the planar square lattice with nearest-neighbor steps and general i.i.d. weights on the vertices, outside of the class of exactly solvable models. We show how stationary cocycles are constructed from queueing fixed points and how these cocycles characterize the limit shape, yield existence of Busemann functions in directions where the shape has some regularity, describe the direction of the competition interface, and answer questions on existence, uniqueness, and coalescence of directional semi-infinite geodesics, and on nonexistence of doubly infinite geodesics.

==> macros.tex <==
%    If you need symbols beyond the basic set, uncomment this command.
\usepackage{amssymb}

%    If your article includes graphics, uncomment this command.
%\usepackage{graphicx}

%    If the article includes commutative diagrams, ...
%\usepackage[cmtip,all]{xy}

%    Include other referenced packages here.
\usepackage{amsmath,amsthm,tikz,mathrsfs,pgfplots,enumerate}
\usepackage{bm}
%\usepackage{subfiles}
\RequirePackage[numbers,sort&compress]{natbib}
\RequirePackage{color}
\definecolor{my-link}{rgb}{0.5,0.0,0.0}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.0,0.5,0.0}
\RequirePackage[colorlinks, urlcolor=my-blue,linkcolor=my-link,citecolor=my-green]{hyperref}
%\usepackage[colorlinks=true]{hyperref}
%the link colors were adjusted slightly so that they print nicely even in black and white

%\usepackage[left=1in,top=1in,right=1in,bottom=1in]{geometry}
%\usepackage[left=1.5in,top=1.5in,right=1.5in,bottom=1.4in]{geometry}

%\linespread{1.1}     %this works nicely to produce a more readable cropped 2-1
\usepackage{scalerel}    %%%%  used first for scaling \bullet  
\usepackage{stmaryrd}   %%%% for integer interval notation 
\usepackage{mathabx}   %% made \widecheck work  
\usepackage{hyphenat}

\usepackage{afterpage}

\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}

\renewcommand{\bibsection}{\section*{\refname}}

%Ivan's packages
\usepackage{bbm}
%\usepackage{amsfonts,amsbsy, amscd}
%\usepackage{graphicx,psfrag,subfigure} %,url}
%\usepackage{cite}
%\usepackage[DIV13]{typearea}
%\usepackage{comment}
%\usepackage{caption}
%\usepackage{setspace}
%\usepackage{float}

%\usepackage{chapterbib}
%\usepackage{minitoc}
%\usepackage{appendix}
%\setcounter{secnumdepth}{3}

%\usepackage{filemod} 
%\date{Last modified on \today\ at\ \filemodprinttime{\jobname}}
%\date{December 05, 2016}



%    Update the information and uncomment if AMS is not the copyright
%    holder.
%\copyrightinfo{2009}{American Mathematical Society}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{formal}[theorem]{Critical point derivation}
\newtheorem{experiment}[theorem]{Experimental Result}
\newtheorem{clam}[theorem]{Claim}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
%\newtheorem{xca}[theorem]{Exercise}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conj}[theorem]{Conjecture}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newenvironment{remarks}{\begin{remark}\normalfont}{\end{remark}}
\newtheorem{quest}{Question}


\allowdisplaybreaks[1]
\numberwithin{figure}{section}
\numberwithin{equation}{section}

\newcommand\docname[2]{#2}

\let\LATEXindex\index % save old definition to prevent recursion
\renewcommand\index[1]{\LATEXindex{#1|docname{\jobname}}}
\makeindex

%%%%%%%%%%%%%%%%%%%%
%Firas' macros
%%%%%%%%%%%%%%%%%%%%
\definecolor{sussexg}{rgb}{0,0.7,0.7}
\definecolor{sussexp}{rgb}{0.4,0,0.4}
\definecolor{sussexb}{rgb}{0.4,0.4,0.7}
\definecolor{mygray}{rgb}{0.75,0.75,0.75}


\newcommand{\E}{\mathbb{E}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cT}{\mathcal{T}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\e}{\varepsilon}
\newcommand{\kS}{\mathfrak{S}}
\def\w{\omega}
\def\Bavg{\overline B}
\def\Gbar{\overline G}
\def\cid{\xi^*}

\def\esssup{\mathop{\mathrm{ess\,sup}}}
\def\range{\mathcal R}
\def\Uset{\mathcal U}
\def\riUset{\Uset^\circ}

\font \mymathbb = bbold10 at 11pt
\newcommand{\one}{\mbox{\mymathbb{1}}}    %indicator function

\def\thick{2pt}



%%%%%%%%%%%%%%%%%%%%
%Timo's macros
%%%%%%%%%%%%%%%%%%%%
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\nn}{\nonumber}
\providecommand{\abs}[1]{\vert#1\vert}
\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 
\newcommand{\ce}[1]{\lceil{#1}\rceil}
\def\cC{\mathcal{C}}  \def\cD{\mathcal{D}}
\def\cR{\mathcal{R}}
\def\cU{\mathcal{U}}
\def\cK{\mathcal{K}}
\def\cX{\mathcal{X}}\def\cY{\mathcal{Y}}\def\cZ{\mathcal{Z}}
\def\bE{\mathbb{E}} \def\bL{\mathbb{L}}
\def\uvec{\mathbf{u}}\def\vvec{\mathbf{v}}
\def\wvec{\mathbf{w}}
\def\ind{\mathbf{1}}
\def\ddd{\displaystyle} 
\def\Vvv{{\rm\mathbb{V}ar}}  \def\Cvv{{\rm\mathbb{C}ov}} 
\def\wt{\widetilde}  \def\wh{\widehat} \def\wb{\overline} \def\wc{\widecheck}
\def\north{S_{\mathcal N}}  \def\south{S_{\mathcal S}}  \def\east{S_{\mathcal E}}  
\def\west{S_{\mathcal W}}  
\def\OSP{(\Omega, \kS, \P)}
\def\Gpl{G}
\def\Gpp{G}
\def\gpp{g_{\text{\rm pp}}}
\def\gpl{g_{\text{\rm pl}}}  
\def\B{{B}}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\conv}{co}   %convex hull  
\def\sigmawc{\wc\sigma}   %sigma check (needed version that doesn't start \w...  
\def\loexp{\chi}  %longitudinal exponent
\def\trexp{\zeta}  %transverse exponent
\def\deq{\overset{d}=} 
\def\qedex{\hfill$\triangle$} 
\def\bincr{B}   \def\tincr{t}   \def\Iincr{I}
\def\Xw{X}  %another letter for a weight 
\def\Yw{Y}  %another letter for a weight 
\def\ul{\underline}  
\def\exitt{\tau} %exit time from axis 
\def\Gppo{{{}^o\Gpp}}
\newcommand\bbullet{{\raisebox{0.5pt}{\scaleobj{0.6}{\bullet}}}} %% looks good for paths x_\bbullet 
\newcommand\brbullet{{\raisebox{-1pt}{\scaleobj{0.5}{\bullet}}}} %%  for subscript paths x_\bbullet   need negative raise 
\newcommand\cbullet{{\raisebox{1pt}{\scaleobj{0.6}{\bullet}}}}
\newcommand\dbullet{{\scaleobj{0.7}{\bullet}}}   % same as \bbullet but without shift up


%%%%%%%%%%%%%%%%%%%%
%Ivan's macros
%%%%%%%%%%%%%%%%%%%%
\newcommand{\bflambda}{\ensuremath{\bar{\lambda}}}
\newcommand{\bfmu}{\ensuremath{\bar{\mu}}}
\newcommand{\bfnu}{\ensuremath{\bar{\nu}}}
\newcommand{\I}{{\rm i}}
\newcommand{\Id}{\mathbbm{1}}
\newcommand{\Or}{\mathcal{O}}
%\newcommand{\e}[0]{\varepsilon}
\newcommand{\BesselK}{\ensuremath{\mathrm{K}}}
\newcommand{\EE}{\ensuremath{\mathbb{E}}}
\newcommand{\PP}{\ensuremath{\mathbb{P}}}
%\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
%\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Rplus}{\ensuremath{\mathbb{R}_{+}}}
\newcommand{\Zgzero}{\ensuremath{\mathbb{Z}_{>0}}}
\newcommand{\Zgeqzero}{\ensuremath{\mathbb{Z}_{\geq 0}}}
\newcommand{\Zleqzero}{\ensuremath{\mathbb{Z}_{\leq 0}}}
%\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\Y}{\ensuremath{\mathbb{Y}}}
\newcommand{\M}{\ensuremath{\mathbf{M}}}
\newcommand{\MM}{\ensuremath{\mathbf{MM}}}
\newcommand{\W}[1]{\ensuremath{\mathbf{W}}_{(#1)}}
\newcommand{\WM}[1]{\ensuremath{\mathbf{WM}}_{(#1)}}
\newcommand{\Zsd}{\ensuremath{\mathbf{Z}}}
\newcommand{\Fsd}{\ensuremath{\mathbf{F}}}
\newcommand{\Usd}{\ensuremath{\mathbf{U}}}
\newcommand{\Sym}{\ensuremath{\mathrm{Sym}}}
\newcommand{\Gdist}{\ensuremath{\mathrm{Gamma}}}
\newcommand{\LogGdist}{\ensuremath{\log\Gamma}}
\newcommand{\Hi}{\ensuremath{\mathcal{H}}}
\newcommand{\Res}[1]{\underset{{#1}}{\mathrm{Res}}}
\newcommand{\ta}[0]{\varphi}
\newcommand{\T}{\mathbb{T}}
\newcommand{\la}{\lambda}
\newcommand{\ga}{\gamma}
\newcommand{\ep}{\epsilon}
\newcommand{\RR}{\mathbb{R}_+\times\mathbb{R}}

\renewcommand{\d}{\mathrm d}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\Ai}{Ai} \DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator*{\var}{Var}
\DeclareMathOperator*{\sgn}{sgn}




%%%%%%%%%%%%%%%%%%%%
%Jack's macros
%%%%%%%%%%%%%%%%%%%%

%commands
\newcommand{\prob}{\mathbf{P}}
%\newcommand{\Z}{\mathbb{Z}}
\newcommand{\cE}{\mathcal{E}}
%\newcommand{\cB}{\mathcal{B}}
%\newcommand{\cN}{\mathcal{N}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbR}{\mathbb{R}}


